Cell Type Identification from Single-Cell Transcriptomic Data via Semi-supervised Learning

Cell type identification from single-cell transcriptomic data is a common goal of single-cell RNA sequencing (scRNAseq) data analysis. Neural networks have been employed to identify cell types from scRNAseq data with high performance. However, it requires a large mount of individual cells with accurate and unbiased annotated types to build the identification models. Unfortunately, labeling the scRNAseq data is cumbersome and time-consuming as it involves manual inspection of marker genes. To overcome this challenge, we propose a semi-supervised learning model to use unlabeled scRNAseq cells and limited amount of labeled scRNAseq cells to implement cell identification. Firstly, we transform the scRNAseq cells to "gene sentences", which is inspired by similarities between natural language system and gene system. Then genes in these sentences are represented as gene embeddings to reduce data sparsity. With these embeddings, we implement a semi-supervised learning model based on recurrent convolutional neural networks (RCNN), which includes a shared network, a supervised network and an unsupervised network. The proposed model is evaluated on macosko2015, a large scale single-cell transcriptomic dataset with ground truth of individual cell types. It is observed that the proposed model is able to achieve encouraging performance by learning on very limited amount of labeled scRNAseq cells together with a large number of unlabeled scRNAseq cells.

==> Data.tex <==

Single-cell genomics can characterize cell identity and function, but limitations of ease and scale have prevented its broad application. Macosko \textit{et al.}~\cite{macosko2015highly} proposed Drop-seq, a strategy for quickly profiling thousands of individual cells by separating them into nanoliter-sized aqueous droplets, associating a different barcode with each cell’s RNAs, and sequencing them all together. We employed the datasets including 44,825 mouse retinal cells and identified 39 transcriptionally distinct cell populations\footnote{https://github.com/olgabot/macosko2015}. The retina dataset with 24,760 genes contains 12 classes including rods, cones, muller glia, astrocytes,  fibroblasts, vascular endothelium, pericytes, microglia, retinal ganglion, bipolar, horizontal, and amacrine. The cell distribution is shown in Figure~\ref{Fig2_cell}. Most of the classes are divisible into discrete types—a total currently estimated at about 100—but well under half of these types possess known, distinguishing molecular markers.

\begin{figure} [!h]
	\includegraphics[width=\linewidth]{Figure/cell_dis.pdf}
	\caption{Cell distribution in different subtypes. }
	\label{Fig2_cell}
\end{figure}





